On Quantum Simulation Of Cosmic Inflation

In this paper, we generalize Jordan-Lee-Preskill, an algorithm for simulating flat-space quantum field theories, to 3+1 dimensional inflationary spacetime. The generalized algorithm contains the encoding treatment, the initial state preparation, the inflation process, and the quantum measurement of cosmological observables at late time. The algorithm is helpful for obtaining predictions of cosmic non-Gaussianities, serving as useful benchmark problems for quantum devices, and checking assumptions made about interacting vacuum in the inflationary perturbation theory. Components of our work also include a detailed discussion about the lattice regularization of the cosmic perturbation theory, a detailed discussion about the in-in formalism, a discussion about encoding using the HKLL-type formula that might apply for both dS and AdS spacetimes, a discussion about bounding curvature perturbations, a description of the three-party Trotter simulation algorithm for time-dependent Hamiltonians, a ground state projection algorithm for simulating gapless theories, a discussion about the quantum-extended Church-Turing Thesis, and a discussion about simulating cosmic reheating in quantum devices.

==> inflation <==
@article{Chatrchyan:2020syc,
    author = {Chatrchyan, Aleksandr and Geier, Kevin T. and Oberthaler, Markus K. and Berges, J\"urgen and Hauke, Philipp},
    title = "{Analog reheating of the early universe in the laboratory}",
    eprint = "2008.02290",
    archivePrefix = "arXiv",
    primaryClass = "cond-mat.quant-gas",
    month = "8",
    year = "2020"
}

@article{Guth:1980zm,
    author = "Guth, Alan H.",
    editor = "Fang, Li-Zhi and Ruffini, R.",
    title = "{The Inflationary Universe: A Possible Solution to the Horizon and Flatness Problems}",
    reportNumber = "SLAC-PUB-2576",
    doi = "10.1103/PhysRevD.23.347",
    journal = "Adv. Ser. Astrophys. Cosmol.",
    volume = "3",
    pages = "139--148",
    year = "1987"
}

@article{Linde:1981mu,
    author = "Linde, Andrei D.",
    editor = "Fang, Li-Zhi and Ruffini, R.",
    title = "{A New Inflationary Universe Scenario: A Possible Solution of the Horizon, Flatness, Homogeneity, Isotropy and Primordial Monopole
    Problems}",
    reportNumber = "LEBEDEV-81-229",
    doi = "10.1016/0370-2693(82)91219-9",
    journal = "Adv. Ser. Astrophys. Cosmol.",
    volume = "3",
    pages = "149--153",
    year = "1987"
}

@article{Albrecht:1982wi,
    author = "Albrecht, Andreas and Steinhardt, Paul J.",
    editor = "Fang, Li-Zhi and Ruffini, R.",
    title = "{Cosmology for Grand Unified Theories with Radiatively Induced Symmetry Breaking}",
    reportNumber = "UPR-0185T",
    doi = "10.1103/PhysRevLett.48.1220",
    journal = "Adv. Ser. Astrophys. Cosmol.",
    volume = "3",
    pages = "158--161",
    year = "1987"
}

@article{Starobinsky:1980te,
    author = "Starobinsky, Alexei A.",
    editor = "Khalatnikov, I.M. and Mineev, V.P.",
    title = "{A New Type of Isotropic Cosmological Models Without Singularity}",
    doi = "10.1016/0370-2693(80)90670-X",
    journal = "Adv. Ser. Astrophys. Cosmol.",
    volume = "3",
    pages = "130--133",
    year = "1987"
}

@article{Sato:1980yn,
    author = "Sato, K.",
    title = "{First Order Phase Transition of a Vacuum and Expansion of the Universe}",
    reportNumber = "NORDITA-80-29",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "195",
    pages = "467--479",
    year = "1981"
}


@article{Mukhanov:1981xt,
    author = "Mukhanov, Viatcheslav F. and Chibisov, G. V.",
    title = "{Quantum Fluctuations and a Nonsingular Universe}",
    journal = "JETP Lett.",
    volume = "33",
    pages = "532--535",
    year = "1981"
}

@article{Starobinsky:1982ee,
    author = "Starobinsky, Alexei A.",
    title = "{Dynamics of Phase Transition in the New Inflationary Universe Scenario and Generation of Perturbations}",
    doi = "10.1016/0370-2693(82)90541-X",
    journal = "Phys. Lett. B",
    volume = "117",
    pages = "175--178",
    year = "1982"
}

@article{Guth:1982ec,
    author = "Guth, Alan H. and Pi, S.Y.",
    title = "{Fluctuations in the New Inflationary Universe}",
    doi = "10.1103/PhysRevLett.49.1110",
    journal = "Phys. Rev. Lett.",
    volume = "49",
    pages = "1110--1113",
    year = "1982"
}

@article{Bardeen:1983qw,
    author = "Bardeen, James M. and Steinhardt, Paul J. and Turner, Michael S.",
    title = "{Spontaneous Creation of Almost Scale - Free Density Perturbations in an Inflationary Universe}",
    reportNumber = "UPR-0202T, EFI-83-13-CHICAGO",
    doi = "10.1103/PhysRevD.28.679",
    journal = "Phys. Rev. D",
    volume = "28",
    pages = "679",
    year = "1983"
}

@article{Mukhanov:1990me,
    author = "Mukhanov, Viatcheslav F. and Feldman, H.A. and Brandenberger, Robert H.",
    title = "{Theory of cosmological perturbations. Part 1. Classical perturbations. Part 2. Quantum theory of perturbations. Part 3. Extensions}",
    reportNumber = "BROWN-HET-796, BROWN-HET-800, BROWN-HET-780",
    doi = "10.1016/0370-1573(92)90044-Z",
    journal = "Phys. Rept.",
    volume = "215",
    pages = "203--333",
    year = "1992"
}

@book{Linde:2005ht,
    author = "Linde, Andrei D.",
    title = "{Particle physics and inflationary cosmology}",
    eprint = "hep-th/0503203",
    archivePrefix = "arXiv",
    volume = "5",
    year = "1990"
}

@article{Malik:2008im,
    author = "Malik, Karim A. and Wands, David",
    title = "{Cosmological perturbations}",
    eprint = "0809.4944",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph",
    doi = "10.1016/j.physrep.2009.03.001",
    journal = "Phys. Rept.",
    volume = "475",
    pages = "1--51",
    year = "2009"
}

@inproceedings{Baumann:2009ds,
    author = "Baumann, Daniel",
    title = "{Inflation}",
    booktitle = "{Theoretical Advanced Study Institute in Elementary Particle Physics}: {Physics of the Large and the Small}",
    eprint = "0907.5424",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "TASI-2009",
    doi = "10.1142/9789814327183\_0010",
    pages = "523--686",
    year = "2011"
}

@article{Chen:2010xka,
    author = "Chen, Xingang",
    title = "{Primordial Non-Gaussianities from Inflation Models}",
    eprint = "1002.1416",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1155/2010/638979",
    journal = "Adv. Astron.",
    volume = "2010",
    pages = "638979",
    year = "2010"
}


@book{Baumann:2014nda,
    author = "Baumann, Daniel and McAllister, Liam",
    title = "{Inflation and String Theory}",
    eprint = "1404.2601",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1017/CBO9781316105733",
    isbn = "978-1-107-08969-3, 978-1-316-23718-2",
    publisher = "Cambridge University Press",
    series = "Cambridge Monographs on Mathematical Physics",
    month = "5",
    year = "2015"
}

@article{Wang:2013zva,
    author = "Wang, Yi",
    title = "{Inflation, Cosmic Perturbations and Non-Gaussianities}",
    eprint = "1303.1523",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/0253-6102/62/1/19",
    journal = "Commun. Theor. Phys.",
    volume = "62",
    pages = "109--166",
    year = "2014"
}

@article{Abbott:1982hn,
    author = "Abbott, L.F. and Farhi, Edward and Wise, Mark B.",
    title = "{Particle Production in the New Inflationary Cosmology}",
    reportNumber = "MIT-CTP-983",
    doi = "10.1016/0370-2693(82)90867-X",
    journal = "Phys. Lett. B",
    volume = "117",
    pages = "29",
    year = "1982"
}

@article{Dolgov:1982th,
    author = "Dolgov, A.D. and Linde, Andrei D.",
    title = "{Baryon Asymmetry in Inflationary Universe}",
    reportNumber = "ITEP-78-1982",
    doi = "10.1016/0370-2693(82)90292-1",
    journal = "Phys. Lett. B",
    volume = "116",
    pages = "329",
    year = "1982"
}

@article{Albrecht:1982mp,
    author = "Albrecht, Andreas and Steinhardt, Paul J. and Turner, Michael S. and Wilczek, Frank",
    title = "{Reheating an Inflationary Universe}",
    reportNumber = "UPR-0189T, EFI-82-09-CHICAGO",
    doi = "10.1103/PhysRevLett.48.1437",
    journal = "Phys. Rev. Lett.",
    volume = "48",
    pages = "1437",
    year = "1982"
}


@article{Traschen:1990sw,
    author = "Traschen, Jennie H. and Brandenberger, Robert H.",
    title = "{Particle Production During Out-of-equilibrium Phase Transitions}",
    reportNumber = "BROWN-HET-731",
    doi = "10.1103/PhysRevD.42.2491",
    journal = "Phys. Rev. D",
    volume = "42",
    pages = "2491--2504",
    year = "1990"
}

@article{Kofman:1994rk,
    author = "Kofman, Lev and Linde, Andrei D. and Starobinsky, Alexei A.",
    title = "{Reheating after inflation}",
    eprint = "hep-th/9405187",
    archivePrefix = "arXiv",
    reportNumber = "UH-IFA-94-35, SU-ITP-94-13, YITP-U-94-15",
    doi = "10.1103/PhysRevLett.73.3195",
    journal = "Phys. Rev. Lett.",
    volume = "73",
    pages = "3195--3198",
    year = "1994"
}

@article{Shtanov:1994ce,
    author = "Shtanov, Y. and Traschen, Jennie H. and Brandenberger, Robert H.",
    title = "{Universe reheating after inflation}",
    eprint = "hep-ph/9407247",
    archivePrefix = "arXiv",
    reportNumber = "BROWN-HET-957",
    doi = "10.1103/PhysRevD.51.5438",
    journal = "Phys. Rev. D",
    volume = "51",
    pages = "5438--5455",
    year = "1995"
}

@article{Kuzmin:1985mm,
    author = "Kuzmin, V.A. and Rubakov, V.A. and Shaposhnikov, M.E.",
    title = "{On the Anomalous Electroweak Baryon Number Nonconservation in the Early Universe}",
    reportNumber = "IC/85/8",
    doi = "10.1016/0370-2693(85)91028-7",
    journal = "Phys. Lett. B",
    volume = "155",
    pages = "36",
    year = "1985"
}

@article{Sakharov:1967dj,
    author = "Sakharov, A.D.",
    title = "{Violation of CP Invariance, C asymmetry, and baryon asymmetry of the universe}",
    doi = "10.1070/PU1991v034n05ABEH002497",
    journal = "Sov. Phys. Usp.",
    volume = "34",
    number = "5",
    pages = "392--393",
    year = "1991"
}

@article{Shaposhnikov:1987tw,
    author = "Shaposhnikov, M.E.",
    title = "{Baryon Asymmetry of the Universe in Standard Electroweak Theory}",
    doi = "10.1016/0550-3213(87)90127-1",
    journal = "Nucl. Phys. B",
    volume = "287",
    pages = "757--775",
    year = "1987"
}

@article{Cohen:1993nk,
    author = "Cohen, Andrew G. and Kaplan, D.B. and Nelson, A.E.",
    title = "{Progress in electroweak baryogenesis}",
    eprint = "hep-ph/9302210",
    archivePrefix = "arXiv",
    reportNumber = "UCSD-PTH-93-02, BUHEP-93-4",
    doi = "10.1146/annurev.ns.43.120193.000331",
    journal = "Ann. Rev. Nucl. Part. Sci.",
    volume = "43",
    pages = "27--70",
    year = "1993"
}

@article{Riess:1998cb,
    author = "Riess, Adam G. and others",
    collaboration = "Supernova Search Team",
    title = "{Observational evidence from supernovae for an accelerating universe and a cosmological constant}",
    eprint = "astro-ph/9805201",
    archivePrefix = "arXiv",
    doi = "10.1086/300499",
    journal = "Astron. J.",
    volume = "116",
    pages = "1009--1038",
    year = "1998"
}

@article{Carroll:2000fy,
    author = "Carroll, Sean M.",
    title = "{The Cosmological constant}",
    eprint = "astro-ph/0004075",
    archivePrefix = "arXiv",
    reportNumber = "EFI-2000-13",
    doi = "10.12942/lrr-2001-1",
    journal = "Living Rev. Rel.",
    volume = "4",
    pages = "1",
    year = "2001"
}

@article{Peebles:2002gy,
    author = "Peebles, P.J.E. and Ratra, Bharat",
    editor = "Hsu, Jong-Ping and Fine, D.",
    title = "{The Cosmological Constant and Dark Energy}",
    eprint = "astro-ph/0207347",
    archivePrefix = "arXiv",
    reportNumber = "KSUPT-02-3",
    doi = "10.1103/RevModPhys.75.559",
    journal = "Rev. Mod. Phys.",
    volume = "75",
    pages = "559--606",
    year = "2003"
}

@article{Maldacena:2002vr,
    author = "Maldacena, Juan Martin",
    title = "{Non-Gaussian features of primordial fluctuations in single field inflationary models}",
    eprint = "astro-ph/0210603",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2003/05/013",
    journal = "JHEP",
    volume = "05",
    pages = "013",
    year = "2003"
}


@article{Chen:2006nt,
    author = "Chen, Xingang and Huang, Min-xin and Kachru, Shamit and Shiu, Gary",
    title = "{Observational signatures and non-Gaussianities of general single field inflation}",
    eprint = "hep-th/0605045",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-11840, MAD-TH-06-3, UFIFT-HEP-06-9, SU-ITP-06-12, CU-TP-1147",
    doi = "10.1088/1475-7516/2007/01/002",
    journal = "JCAP",
    volume = "01",
    pages = "002",
    year = "2007"
}

@article{Cheung:2007st,
    author = "Cheung, Clifford and Creminelli, Paolo and Fitzpatrick, A.Liam and Kaplan, Jared and Senatore, Leonardo",
    title = "{The Effective Field Theory of Inflation}",
    eprint = "0709.0293",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "IC-2007-032",
    doi = "10.1088/1126-6708/2008/03/014",
    journal = "JHEP",
    volume = "03",
    pages = "014",
    year = "2008"
}

@article{Weinberg:2008hq,
    author = "Weinberg, Steven",
    title = "{Effective Field Theory for Inflation}",
    eprint = "0804.4291",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "UTTG-01-08",
    doi = "10.1103/PhysRevD.77.123541",
    journal = "Phys. Rev. D",
    volume = "77",
    pages = "123541",
    year = "2008"
}

@article{Chen:2009zp,
    author = "Chen, Xingang and Wang, Yi",
    title = "{Quasi-Single Field Inflation and Non-Gaussianities}",
    eprint = "0911.3380",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2010/04/027",
    journal = "JCAP",
    volume = "04",
    pages = "027",
    year = "2010"
}

@inproceedings{Witten:2001kn,
    author = "Witten, Edward",
    title = "{Quantum gravity in de Sitter space}",
    booktitle = "{Strings 2001: International Conference}",
    eprint = "hep-th/0106109",
    archivePrefix = "arXiv",
    month = "6",
    year = "2001"
}

@article{Strominger:2001pn,
    author = "Strominger, Andrew",
    title = "{The dS / CFT correspondence}",
    eprint = "hep-th/0106113",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2001/10/034",
    journal = "JHEP",
    volume = "10",
    pages = "034",
    year = "2001"
}

@inproceedings{Maloney:2002rr,
    author = "Maloney, Alexander and Silverstein, Eva and Strominger, Andrew",
    title = "{De Sitter space in noncritical string theory}",
    booktitle = "{Workshop on Conference on the Future of Theoretical Physics and Cosmology in Honor of Steven Hawking's 60th Birthday}",
    eprint = "hep-th/0205316",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-9228, HUTP-02-A019",
    pages = "570--591",
    month = "5",
    year = "2002"
}

@article{Alishahiha:2004md,
    author = "Alishahiha, Mohsen and Karch, Andreas and Silverstein, Eva and Tong, David",
    editor = "Allen, R.E. and Nanopoulos, Dimitri V. and Pope, C.N.",
    title = "{The dS/dS correspondence}",
    eprint = "hep-th/0407125",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-10540, SU-ITP-04-29, IPM-P-2004-31, MIT-CTP-3512, UW-PT-04-07",
    doi = "10.1063/1.1848341",
    journal = "AIP Conf. Proc.",
    volume = "743",
    number = "1",
    pages = "393--409",
    year = "2004"
}

@article{Kachru:2003aw,
    author = "Kachru, Shamit and Kallosh, Renata and Linde, Andrei D. and Trivedi, Sandip P.",
    title = "{De Sitter vacua in string theory}",
    eprint = "hep-th/0301240",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-9630, SU-ITP-03-01, TIFR-TH-03-03",
    doi = "10.1103/PhysRevD.68.046005",
    journal = "Phys. Rev. D",
    volume = "68",
    pages = "046005",
    year = "2003"
}

@article{Arkani-Hamed:2015bza,
    author = "Arkani-Hamed, Nima and Maldacena, Juan",
    title = "{Cosmological Collider Physics}",
    eprint = "1503.08043",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "3",
    year = "2015"
}

@article{preskill2018quantum,
  title={Quantum Computing in the NISQ era and beyond},
  author={Preskill, John},
  journal={Quantum},
  volume={2},
  pages={79},
  year={2018},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}

@article{arute2019quantum,
  title={Quantum supremacy using a programmable superconducting processor},
  author={Arute, Frank and Arya, Kunal and Babbush, Ryan and Bacon, Dave and Bardin, Joseph C and Barends, Rami and Biswas, Rupak and Boixo, Sergio
  and Brandao, Fernando GSL and Buell, David A and others},
  journal={Nature},
  volume={574},
  number={7779},
  pages={505--510},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{Jordan:2011ne,
    author = "Jordan, Stephen P. and Lee, Keith S.M. and Preskill, John",
    title = "{Quantum Algorithms for Quantum Field Theories}",
    eprint = "1111.3633",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    doi = "10.1126/science.1217069",
    journal = "Science",
    volume = "336",
    pages = "1130--1133",
    year = "2012"
}

@article{Jordan:2011ci,
    author = "Jordan, Stephen P. and Lee, Keith S.M. and Preskill, John",
    title = "{Quantum Computation of Scattering in Scalar Quantum Field Theories}",
    eprint = "1112.4833",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    journal = "Quant. Inf. Comput.",
    volume = "14",
    pages = "1014--1080",
    year = "2014"
}

@article{Preskill:2018fag,
    author = "Preskill, John",
    title = "{Simulating quantum field theory with a quantum computer}",
    eprint = "1811.10085",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    doi = "10.22323/1.334.0024",
    journal = "PoS",
    volume = "LATTICE2018",
    pages = "024",
    year = "2018"
}

@article{jordan2014quantum,
  title={Quantum algorithms for fermionic quantum field theories},
  author={Jordan, Stephen P and Lee, Keith SM and Preskill, John},
  journal={arXiv preprint arXiv:1404.7115},
  year={2014}
}

@article{jordan2018bqp,
  title={BQP-completeness of scattering in scalar quantum field theory},
  author={Jordan, Stephen P and Krovi, Hari and Lee, Keith SM and Preskill, John},
  journal={Quantum},
  volume={2},
  pages={44},
  year={2018},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}

@article{Gary:2009ae,
    author = "Gary, Mirah and Giddings, Steven B. and Penedones, Joao",
    title = "{Local bulk S-matrix elements and CFT singularities}",
    eprint = "0903.4437",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2009-035, NSF-KITP-09-35",
    doi = "10.1103/PhysRevD.80.085005",
    journal = "Phys. Rev. D",
    volume = "80",
    pages = "085005",
    year = "2009"
}

@article{Heemskerk:2009pn,
    author = "Heemskerk, Idse and Penedones, Joao and Polchinski, Joseph and Sully, James",
    title = "{Holography from Conformal Field Theory}",
    eprint = "0907.0151",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "NSF-KITP-09-110",
    doi = "10.1088/1126-6708/2009/10/079",
    journal = "JHEP",
    volume = "10",
    pages = "079",
    year = "2009"
}

@article{Giddings:2009gj,
    author = "Giddings, Steven B. and Porto, Rafael A.",
    title = "{The Gravitational S-matrix}",
    eprint = "0908.0004",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2009-142",
    doi = "10.1103/PhysRevD.81.025002",
    journal = "Phys. Rev. D",
    volume = "81",
    pages = "025002",
    year = "2010"
}

@article{Fitzpatrick:2010zm,
    author = "Fitzpatrick, A.Liam and Katz, Emanuel and Poland, David and Simmons-Duffin, David",
    title = "{Effective Conformal Theory and the Flat-Space Limit of AdS}",
    eprint = "1007.2412",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "BUHET-07-14-10",
    doi = "10.1007/JHEP07(2011)023",
    journal = "JHEP",
    volume = "07",
    pages = "023",
    year = "2011"
}

@article{Fitzpatrick:2011hu,
    author = "Fitzpatrick, A.Liam and Kaplan, Jared",
    title = "{Analyticity and the Holographic S-Matrix}",
    eprint = "1111.6972",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC-PUB-14841",
    doi = "10.1007/JHEP10(2012)127",
    journal = "JHEP",
    volume = "10",
    pages = "127",
    year = "2012"
}

@article{Fitzpatrick:2011dm,
    author = "Fitzpatrick, A.Liam and Kaplan, Jared",
    title = "{Unitarity and the Holographic S-Matrix}",
    eprint = "1112.4845",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC-PUB-14979",
    doi = "10.1007/JHEP10(2012)032",
    journal = "JHEP",
    volume = "10",
    pages = "032",
    year = "2012"
}

@article{Maldacena:2015iua,
    author = "Maldacena, Juan and Simmons-Duffin, David and Zhiboedov, Alexander",
    title = "{Looking for a bulk point}",
    eprint = "1509.03612",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP01(2017)013",
    journal = "JHEP",
    volume = "01",
    pages = "013",
    year = "2017"
}

@article{ElShowk:2011ag,
    author = "El-Showk, Sheer and Papadodimas, Kyriakos",
    title = "{Emergent Spacetime and Holographic CFTs}",
    eprint = "1101.4163",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2012)106",
    journal = "JHEP",
    volume = "10",
    pages = "106",
    year = "2012"
}

@article{Weinberg:2005vy,
    author = "Weinberg, Steven",
    title = "{Quantum contributions to cosmological correlations}",
    eprint = "hep-th/0506236",
    archivePrefix = "arXiv",
    reportNumber = "UTTG-01-05",
    doi = "10.1103/PhysRevD.72.043514",
    journal = "Phys. Rev. D",
    volume = "72",
    pages = "043514",
    year = "2005"
}

@article{Senatore:2009cf,
    author = "Senatore, Leonardo and Zaldarriaga, Matias",
    title = "{On Loops in Inflation}",
    eprint = "0912.2734",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP12(2010)008",
    journal = "JHEP",
    volume = "12",
    pages = "008",
    year = "2010"
}

@article{Senatore:2012nq,
    author = "Senatore, Leonardo and Zaldarriaga, Matias",
    title = "{On Loops in Inflation II: IR Effects in Single Clock Inflation}",
    eprint = "1203.6354",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC-PUB-15860",
    doi = "10.1007/JHEP01(2013)109",
    journal = "JHEP",
    volume = "01",
    pages = "109",
    year = "2013"
}

@article{Pimentel:2012tw,
    author = "Pimentel, Guilherme L. and Senatore, Leonardo and Zaldarriaga, Matias",
    title = "{On Loops in Inflation III: Time Independence of zeta in Single Clock Inflation}",
    eprint = "1203.6651",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP07(2012)166",
    journal = "JHEP",
    volume = "07",
    pages = "166",
    year = "2012"
}

@article{Fang:1980wi,
    author = "Fang, L.Z.",
    title = "{Entropy Generation in the Early Universe by Dissipative Processes Near the Higgs' Phase Transitions}",
    reportNumber = "ITP-SB-80-30",
    doi = "10.1016/0370-2693(80)90421-9",
    journal = "Phys. Lett. B",
    volume = "95",
    pages = "154--156",
    year = "1980"
}

@article{Chen:2020tes,
    author = "Chen, Yiming and Gorbenko, Victor and Maldacena, Juan",
    title = "{Bra-ket wormholes in gravitationally prepared states}",
    eprint = "2007.16091",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "7",
    year = "2020"
}

@article{Hartman:2020khs,
    author = "Hartman, Thomas and Jiang, Yikun and Shaghoulian, Edgar",
    title = "{Islands in cosmology}",
    eprint = "2008.01022",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "8",
    year = "2020"
}

@article{Dong:2018cuv,
    author = "Dong, Xi and Silverstein, Eva and Torroba, Gonzalo",
    title = "{De Sitter Holography and Entanglement Entropy}",
    eprint = "1804.08623",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP07(2018)050",
    journal = "JHEP",
    volume = "07",
    pages = "050",
    year = "2018"
}

@article{Lewkowycz:2019xse,
    author = "Lewkowycz, Aitor and Liu, Junyu and Silverstein, Eva and Torroba, Gonzalo",
    title = "{$ T\overline{T} $ and EE, with implications for (A)dS subregion encodings}",
    eprint = "1909.13808",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CALT-TH-2019--031",
    doi = "10.1007/JHEP04(2020)152",
    journal = "JHEP",
    volume = "04",
    pages = "152",
    year = "2020"
}

@article{Bunch:1978yq,
    author = "Bunch, T.S. and Davies, P.C.W.",
    title = "{Quantum Field Theory in de Sitter Space: Renormalization by Point Splitting}",
    doi = "10.1098/rspa.1978.0060",
    journal = "Proc. Roy. Soc. Lond. A",
    volume = "A360",
    pages = "117--134",
    year = "1978"
}

@article{mcardle2020quantum,
  title={Quantum computational chemistry},
  author={McArdle, Sam and Endo, Suguru and Aspuru-Guzik, Alan and Benjamin, Simon C and Yuan, Xiao},
  journal={Reviews of Modern Physics},
  volume={92},
  number={1},
  pages={015003},
  year={2020},
  publisher={APS}
}

@article{Liu:2020eoa,
    author = "Liu, Junyu and Xin, Yuan",
    title = "{Quantum simulation of quantum field theories as quantum chemistry}",
    eprint = "2004.13234",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CALT-TH-2020-009",
    month = "4",
    year = "2020"
}


@article{Easther:2001fi,
    author = "Easther, Richard and Greene, Brian R. and Kinney, William H. and Shiu, Gary",
    title = "{Inflation as a probe of short distance physics}",
    eprint = "hep-th/0104102",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.64.103502",
    journal = "Phys. Rev. D",
    volume = "64",
    pages = "103502",
    year = "2001"
}

@article{Jiang:2016nok,
    author = "Jiang, Hongliang and Wang, Yi and Zhou, Siyi",
    title = "{On the initial condition of inflationary fluctuations}",
    eprint = "1601.01179",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2016/04/041",
    journal = "JCAP",
    volume = "04",
    pages = "041",
    year = "2016"
}

@article{Lewis:2019oyx,
    author = "Lewis, Adam G.M. and Vidal, Guifr?,
    title = "{Classical Simulations of Quantum Field Theory in Curved Spacetime I: Fermionic Hawking-Hartle Vacua from a Staggered Lattice Scheme}",
    eprint = "1911.12978",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    month = "11",
    year = "2019"
}

@article{Burgess:2009bs,
    author = "Burgess, C.P. and Leblond, L. and Holman, R. and Shandera, S.",
    title = "{Super-Hubble de Sitter Fluctuations and the Dynamical RG}",
    eprint = "0912.1608",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2010/03/033",
    journal = "JCAP",
    volume = "03",
    pages = "033",
    year = "2010"
}

@article{Brower:2019kyh,
    author = "Brower, Richard C. and Cogburn, Cameron V. and Fitzpatrick, A. Liam and Howarth, Dean and Tan, Chung-I",
    title = "{Lattice Setup for Quantum Field Theory in AdS$_2$}",
    eprint = "1912.07606",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "12",
    year = "2019"
}

@article{Harlow:2011az,
    author = "Harlow, Daniel and Shenker, Stephen H. and Stanford, Douglas and Susskind, Leonard",
    title = "{Tree-like structure of eternal inflation: A solvable model}",
    eprint = "1110.0496",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SU-ITP-11-47",
    doi = "10.1103/PhysRevD.85.063516",
    journal = "Phys. Rev. D",
    volume = "85",
    pages = "063516",
    year = "2012"
}


@article{Gubser:2016guj,
    author = "Gubser, Steven S. and Knaute, Johannes and Parikh, Sarthak and Samberg, Andreas and Witaszczyk, Przemek",
    title = "{$p$-adic AdS/CFT}",
    eprint = "1605.01061",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "PUPT-2503",
    doi = "10.1007/s00220-016-2813-6",
    journal = "Commun. Math. Phys.",
    volume = "352",
    number = "3",
    pages = "1019--1059",
    year = "2017"
}

@article{Heydeman:2016ldy,
    author = "Heydeman, Matthew and Marcolli, Matilde and Saberi, Ingmar and Stoica, Bogdan",
    title = "{Tensor networks, $p$-adic fields, and algebraic curves: arithmetic and the AdS$_3$/CFT$_2$ correspondence}",
    eprint = "1605.07639",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CALT-TH-2016-013",
    doi = "10.4310/ATMP.2018.v22.n1.a4",
    journal = "Adv. Theor. Math. Phys.",
    volume = "22",
    pages = "93--176",
    year = "2018"
}

@article{Bao:2017iye,
    author = "Bao, Ning and Cao, ChunJun and Carroll, Sean M. and McAllister, Liam",
    title = "{Quantum Circuit Cosmology: The Expansion of the Universe Since the First Qubit}",
    eprint = "1702.06959",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CALT-TH-2017-006",
    month = "2",
    year = "2017"
}

@article{Osborne:2017woa,
    author = "Osborne, Tobias J. and Stiegemann, Deniz E.",
    title = "{Dynamics for holographic codes}",
    eprint = "1706.08823",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    doi = "10.1007/JHEP04(2020)154",
    journal = "JHEP",
    volume = "04",
    pages = "154",
    year = "2020"
}





@article{JPwork,
    author = "Lucia, A and Poulin, D and Preskill, J and Wang, T",
    title = "{working in progress}"
}

@article{Easson:2018qgr,
    author = "Easson, Damien A. and Manton, Tucker",
    title = "{Stable Cosmic Time Crystals}",
    eprint = "1802.03693",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.99.043507",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "4",
    pages = "043507",
    year = "2019"
}

@article{Jacobson:2005bg,
    author = "Jacobson, Ted and Liberati, Stefano and Mattingly, David",
    title = "{Lorentz violation at high energy: Concepts, phenomena and astrophysical constraints}",
    eprint = "astro-ph/0505267",
    archivePrefix = "arXiv",
    doi = "10.1016/j.aop.2005.06.004",
    journal = "Annals Phys.",
    volume = "321",
    pages = "150--196",
    year = "2006"
}

@article{GellMann:1951rw,
    author = "Gell-Mann, Murray and Low, Francis",
    title = "{Bound states in quantum field theory}",
    doi = "10.1103/PhysRev.84.350",
    journal = "Phys. Rev.",
    volume = "84",
    pages = "350--354",
    year = "1951"
}

@article{Hamilton:2005ju,
    author = "Hamilton, Alex and Kabat, Daniel N. and Lifschytz, Gilad and Lowe, David A.",
    title = "{Local bulk operators in AdS/CFT: A Boundary view of horizons and locality}",
    eprint = "hep-th/0506118",
    archivePrefix = "arXiv",
    reportNumber = "BROWN-HET-1448, CU-TP-1130",
    doi = "10.1103/PhysRevD.73.086003",
    journal = "Phys. Rev. D",
    volume = "73",
    pages = "086003",
    year = "2006"
}

@article{Harlow:2018fse,
    author = "Harlow, Daniel",
    title = "{TASI Lectures on the Emergence of Bulk Physics in AdS/CFT}",
    eprint = "1802.01040",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.22323/1.305.0002",
    journal = "PoS",
    volume = "TASI2017",
    pages = "002",
    year = "2018"
}

@article{Martin:2000xs,
    author = "Martin, Jerome and Brandenberger, Robert H.",
    title = "{The TransPlanckian problem of inflationary cosmology}",
    eprint = "hep-th/0005209",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.63.123501",
    journal = "Phys. Rev. D",
    volume = "63",
    pages = "123501",
    year = "2001"
}

@article{kitaev2008wavefunction,
  title={Wavefunction preparation and resampling using a quantum computer},
  author={Kitaev, Alexei and Webb, William A},
  journal={arXiv preprint arXiv:0801.0342},
  year={2008}
}

@article{bunch1974triangular,
  title={Triangular factorization and inversion by fast matrix multiplication},
  author={Bunch, James R and Hopcroft, John E},
  journal={Mathematics of Computation},
  volume={28},
  number={125},
  pages={231--236},
  year={1974}
}

@inproceedings{coppersmith1987matrix,
  title={Matrix multiplication via arithmetic progressions},
  author={Coppersmith, Don and Winograd, Shmuel},
  booktitle={Proceedings of the nineteenth annual ACM symposium on Theory of computing},
  pages={1--6},
  year={1987}
}

@article{childs2019theory,
  title={A theory of Trotter error},
  author={Childs, Andrew M and Su, Yuan and Tran, Minh C and Wiebe, Nathan and Zhu, Shuchen},
  journal={arXiv preprint arXiv:1912.08854},
  year={2019}
}

@article{Gibbons:1977mu,
    author = "Gibbons, G.W. and Hawking, S.W.",
    title = "{Cosmological Event Horizons, Thermodynamics, and Particle Creation}",
    doi = "10.1103/PhysRevD.15.2738",
    journal = "Phys. Rev. D",
    volume = "15",
    pages = "2738--2751",
    year = "1977"
}


@article{Guth:1985ya,
    author = "Guth, Alan H. and Pi, So-Young",
    title = "{The Quantum Mechanics of the Scalar Field in the New Inflationary Universe}",
    reportNumber = "MIT-CTP-1246",
    doi = "10.1103/PhysRevD.32.1899",
    journal = "Phys. Rev. D",
    volume = "32",
    pages = "1899--1920",
    year = "1985"
}

@article{Albrecht:1992kf,
    author = "Albrecht, Andreas and Ferreira, Pedro and Joyce, Michael and Prokopec, Tomislav",
    title = "{Inflation and squeezed quantum states}",
    eprint = "astro-ph/9303001",
    archivePrefix = "arXiv",
    reportNumber = "IMPERIAL-TP-92-93-21",
    doi = "10.1103/PhysRevD.50.4807",
    journal = "Phys. Rev. D",
    volume = "50",
    pages = "4807--4820",
    year = "1994"
}

@article{Lesgourgues:1996jc,
    author = "Lesgourgues, J. and Polarski, David and Starobinsky, Alexei A.",
    title = "{Quantum to classical transition of cosmological perturbations for nonvacuum initial states}",
    eprint = "gr-qc/9611019",
    archivePrefix = "arXiv",
    reportNumber = "LMPT-10-96",
    doi = "10.1016/S0550-3213(97)00224-1",
    journal = "Nucl. Phys. B",
    volume = "497",
    pages = "479--510",
    year = "1997"
}

@article{Kiefer:1998qe,
    author = "Kiefer, Claus and Polarski, David and Starobinsky, Alexei A.",
    title = "{Quantum to classical transition for fluctuations in the early universe}",
    eprint = "gr-qc/9802003",
    archivePrefix = "arXiv",
    reportNumber = "THEP-97-33, FREIBURG-THEP-97-33",
    doi = "10.1142/S0218271898000292",
    journal = "Int. J. Mod. Phys. D",
    volume = "7",
    pages = "455--462",
    year = "1998"
}

@article{Liu:2016aaf,
    author = "Liu, Junyu and Sou, Chon-Man and Wang, Yi",
    title = "{Cosmic Decoherence: Massive Fields}",
    eprint = "1608.07909",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2016)072",
    journal = "JHEP",
    volume = "10",
    pages = "072",
    year = "2016"
}

@article{Almheiri:2014lwa,
    author = "Almheiri, Ahmed and Dong, Xi and Harlow, Daniel",
    title = "{Bulk Locality and Quantum Error Correction in AdS/CFT}",
    eprint = "1411.7041",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SU-ITP-14-30",
    doi = "10.1007/JHEP04(2015)163",
    journal = "JHEP",
    volume = "04",
    pages = "163",
    year = "2015"
}

@article{Dong:2016eik,
    author = "Dong, Xi and Harlow, Daniel and Wall, Aron C.",
    title = "{Reconstruction of Bulk Operators within the Entanglement Wedge in Gauge-Gravity Duality}",
    eprint = "1601.05416",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "NSF-KITP-16-005",
    doi = "10.1103/PhysRevLett.117.021601",
    journal = "Phys. Rev. Lett.",
    volume = "117",
    number = "2",
    pages = "021601",
    year = "2016"
}

@article{Pastawski:2015qua,
    author = "Pastawski, Fernando and Yoshida, Beni and Harlow, Daniel and Preskill, John",
    title = "{Holographic quantum error-correcting codes: Toy models for the bulk/boundary correspondence}",
    eprint = "1503.06237",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP06(2015)149",
    journal = "JHEP",
    volume = "06",
    pages = "149",
    year = "2015"
}

@article{May:2019odp,
    author = "May, Alex and Penington, Geoff and Sorce, Jonathan",
    title = "{Holographic scattering requires a connected entanglement wedge}",
    eprint = "1912.05649",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2020)132",
    journal = "JHEP",
    volume = "20",
    pages = "132",
    year = "2020"
}

@article{low2017optimal,
  title={Optimal Hamiltonian simulation by quantum signal processing},
  author={Low, Guang Hao and Chuang, Isaac L},
  journal={Physical review letters},
  volume={118},
  number={1},
  pages={010501},
  year={2017},
  publisher={APS}
}

@article{Felder:2000hq,
    author = "Felder, Gary N. and Tkachev, Igor",
    title = "{LATTICEEASY: A Program for lattice simulations of scalar fields in an expanding universe}",
    eprint = "hep-ph/0011159",
    archivePrefix = "arXiv",
    reportNumber = "SU-ITP-00-29",
    doi = "10.1016/j.cpc.2008.02.009",
    journal = "Comput. Phys. Commun.",
    volume = "178",
    pages = "929--932",
    year = "2008"
}

@article{Chen:2017fvr,
    author = "Chen, Yu-An and Kapustin, Anton and Radi\v{c}evi\'c, \DJor\dje",
    title = "{Exact bosonization in two spatial dimensions and a new class of lattice gauge theories}",
    eprint = "1711.00515",
    archivePrefix = "arXiv",
    primaryClass = "cond-mat.str-el",
    doi = "10.1016/j.aop.2018.03.024",
    journal = "Annals Phys.",
    volume = "393",
    pages = "234--253",
    year = "2018"
}

@article{Chen:2018nog,
    author = "Chen, Yu-An and Kapustin, Anton",
    title = "{Bosonization in three spatial dimensions and a 2-form gauge theory}",
    eprint = "1807.07081",
    archivePrefix = "arXiv",
    primaryClass = "cond-mat.str-el",
    doi = "10.1103/PhysRevB.100.245127",
    journal = "Phys. Rev. B",
    volume = "100",
    number = "24",
    pages = "245127",
    year = "2019"
}

@article{Chen:2019wlx,
    author = "Chen, Yu-An",
    title = "{Exact bosonization in arbitrary dimensions}",
    eprint = "1911.00017",
    archivePrefix = "arXiv",
    primaryClass = "cond-mat.str-el",
    month = "10",
    year = "2019"
}

@article{wan2020fast,
  title={Fast digital methods for adiabatic state preparation},
  author={Wan, Kianna and Kim, Isaac},
  journal={arXiv preprint arXiv:2004.04164},
  year={2020}
}

@phdthesis{hogarth1996predictability,
  title={Predictability, computability, and spacetime},
  author={Hogarth, Mark},
  year={1996},
  school={University of Cambridge}
}

@article{geroch1986computability,
  title={Computability and physical theories},
  author={Geroch, Robert and Hartle, James B},
  journal={Foundations of Physics},
  volume={16},
  number={6},
  pages={533--550},
  year={1986},
  publisher={Springer}
}

@article{Bouland:2019pvu,
    author = "Bouland, Adam and Fefferman, Bill and Vazirani, Umesh",
    title = "{Computational pseudorandomness, the wormhole growth paradox, and constraints on the AdS/CFT duality}",
    eprint = "1910.14646",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    month = "10",
    year = "2019"
}

@article{Gheorghiu:2020sko,
    author = "Gheorghiu, Alexandru and Hoban, Matty J.",
    title = "{Estimating the entropy of shallow circuit outputs is hard}",
    eprint = "2002.12814",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    month = "2",
    year = "2020"
}

@article{Susskind:2020kti,
    author = "Susskind, Leonard",
    title = "{Horizons Protect Church-Turing}",
    eprint = "2003.01807",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "3",
    year = "2020"
}

@article{Kim:2020cds,
    author = "Kim, Isaac and Tang, Eugene and Preskill, John",
    title = "{The ghost in the radiation: Robust encodings of the black hole interior}",
    eprint = "2003.05451",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP06(2020)031",
    journal = "JHEP",
    volume = "20",
    pages = "031",
    year = "2020"
}

@article{Yoshida:2020wpd,
    author = "Yoshida, Beni",
    title = "{Remarks on Black Hole Complexity Puzzle}",
    eprint = "2005.12491",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "5",
    year = "2020"
}

@article{campbell2019random,
  title={Random compiler for fast Hamiltonian simulation},
  author={Campbell, Earl},
  journal={Physical review letters},
  volume={123},
  number={7},
  pages={070503},
  year={2019},
  publisher={APS}
}

@article{sieberer2019digital,
  title={Digital quantum simulation, Trotter errors, and quantum chaos of the kicked top},
  author={Sieberer, Lukas M and Olsacher, Tobias and Elben, Andreas and Heyl, Markus and Hauke, Philipp and Haake, Fritz and Zoller, Peter},
  journal={npj Quantum Information},
  volume={5},
  number={1},
  pages={1--11},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{chen2020quantum,
  title={Quantum simulation via randomized product formulas: Low gate complexity with accuracy guarantees},
  author={Chen, Chi-Fang and Kueng, Richard and Tropp, Joel A and others},
  journal={arXiv preprint arXiv:2008.11751},
  year={2020}
}

@article{Ashwork,
    author = "Hetherington, V and Milsted, A",
    title = "{private communications}"
}

@article{Danshita:2016xbo,
    author = "Danshita, Ippei and Hanada, Masanori and Tezuka, Masaki",
    title = "{Creating and probing the Sachdev-Ye-Kitaev model with ultracold gases: Towards experimental studies of quantum gravity}",
    eprint = "1606.02454",
    archivePrefix = "arXiv",
    primaryClass = "cond-mat.quant-gas",
    reportNumber = "YITP-16-71",
    doi = "10.1093/ptep/ptx108",
    journal = "PTEP",
    volume = "2017",
    number = "8",
    pages = "083I01",
    year = "2017"
}

@article{Brown:2019hmk,
    author = "Brown, Adam R. and Gharibyan, Hrant and Leichenauer, Stefan and Lin, Henry W. and Nezami, Sepehr and Salton, Grant and Susskind,
    Leonard and Swingle, Brian and Walter, Michael",
    title = "{Quantum Gravity in the Lab: Teleportation by Size and Traversable Wormholes}",
    eprint = "1911.06314",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    month = "11",
    year = "2019"
}

@article{Kobrin:2020xms,
    author = "Kobrin, Bryce and Yang, Zhenbin and Kahanamoku-Meyer, Gregory D. and Olund, Christopher T. and Moore, Joel E. and Stanford, Douglas and
    Yao, Norman Y.",
    title = "{Many-Body Chaos in the Sachdev-Ye-Kitaev Model}",
    eprint = "2002.05725",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "2",
    year = "2020"
}

@article{Landsman:2018jpm,
    author = "Landsman, K.A. and Figgatt, C. and Schuster, T. and Linke, N.M. and Yoshida, B. and Yao, N.Y. and Monroe, C.",
    title = "{Verified Quantum Information Scrambling}",
    eprint = "1806.02807",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    doi = "10.1038/s41586-019-0952-6",
    journal = "Nature",
    volume = "567",
    number = "7746",
    pages = "61--65",
    year = "2019"
}

@article{Babbush:2018mlj,
    author = "Babbush, Ryan and Berry, Dominic W. and Neven, Hartmut",
    title = "{Quantum Simulation of the Sachdev-Ye-Kitaev Model by Asymmetric Qubitization}",
    eprint = "1806.02793",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    doi = "10.1103/PhysRevA.99.040301",
    journal = "Phys. Rev. A",
    volume = "99",
    number = "4",
    pages = "040301",
    year = "2019"
}

@article{Antonini:2019qkt,
    author = "Antonini, Stefano and Swingle, Brian",
    title = "{Cosmology at the end of the world}",
    eprint = "1907.06667",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1038/s41567-020-0909-6",
    journal = "Nature Phys.",
    volume = "16",
    number = "8",
    pages = "881--886",
    year = "2020"
}

@article{Xu:2020shn,
    author = "Xu, Shenglong and Susskind, Leonard and Su, Yuan and Swingle, Brian",
    title = "{A Sparse Model of Quantum Holography}",
    eprint = "2008.02303",
    archivePrefix = "arXiv",
    primaryClass = "cond-mat.str-el",
    month = "8",
    year = "2020"
}

@article{Yuan:2020xmq,
    author = "Yuan, Xiao and Sun, Jinzhao and Liu, Junyu and Zhao, Qi and Zhou, You",
    title = "{Quantum simulation with hybrid tensor networks}",
    eprint = "2007.00958",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    month = "7",
    year = "2020"
}

@article{Wands:1998yp,
    author = "Wands, David",
    title = "{Duality invariance of cosmological perturbation spectra}",
    eprint = "gr-qc/9809062",
    archivePrefix = "arXiv",
    reportNumber = "PU-RCG-98-15",
    doi = "10.1103/PhysRevD.60.023507",
    journal = "Phys. Rev. D",
    volume = "60",
    pages = "023507",
    year = "1999"
}

@article{Finelli:2001sr,
    author = "Finelli, Fabio and Brandenberger, Robert",
    title = "{On the generation of a scale invariant spectrum of adiabatic fluctuations in cosmological models with a contracting phase}",
    eprint = "hep-th/0112249",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.65.103522",
    journal = "Phys. Rev. D",
    volume = "65",
    pages = "103522",
    year = "2002"
}

@article{Khoury:2001wf,
    author = "Khoury, Justin and Ovrut, Burt A. and Steinhardt, Paul J. and Turok, Neil",
    title = "{The Ekpyrotic universe: Colliding branes and the origin of the hot big bang}",
    eprint = "hep-th/0103239",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.64.123522",
    journal = "Phys. Rev. D",
    volume = "64",
    pages = "123522",
    year = "2001"
}

@article{JPtoappear1,
    author = "Liu, Junyu and Preskill, John and Sahinoglu, Burak",
    title = "{Simulating kink scattering in a quantum computer}",
    eprint = "to appear",
    url    = "https://drive.google.com/file/d/1wOrPmO7lfutZlLEj-12JiMUAVg4nOdQr/view"
}

@article{JPtoappear2,
    author = "Milsted, Ashley and Liu, Junyu and Preskill, John and Vidal, Guifre",
    title = "{Simulating kink scattering in tensor networks}",
    eprint = "to appear",
    url    = "https://www.youtube.com/watch?v=9Om--8LsqFw"
}

@article{Witten:1998qj,
    author = "Witten, Edward",
    title = "{Anti-de Sitter space and holography}",
    eprint = "hep-th/9802150",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-98-15",
    doi = "10.4310/ATMP.1998.v2.n2.a2",
    journal = "Adv. Theor. Math. Phys.",
    volume = "2",
    pages = "253--291",
    year = "1998"
}

@article{Aaronson:2005qu,
    author = "Aaronson, Scott",
    title = "{NP-complete problems and physical reality}",
    eprint = "quant-ph/0502072",
    archivePrefix = "arXiv",
    month = "2",
    year = "2005"
}

@article{Bekenstein:1980jp,
    author = "Bekenstein, Jacob D.",
    title = "{A Universal Upper Bound on the Entropy to Energy Ratio for Bounded Systems}",
    reportNumber = "NSF-ITP-80-38",
    doi = "10.1103/PhysRevD.23.287",
    journal = "Phys. Rev. D",
    volume = "23",
    pages = "287",
    year = "1981"
}

@article{Welch:2006va,
    author = "Welch, P.D.",
    title = "{The extent of computation in Malament-Hogarth spacetimes}",
    eprint = "gr-qc/0609035",
    archivePrefix = "arXiv",
    month = "9",
    year = "2006"
}

@article{Hayden:2007cs,
    author = "Hayden, Patrick and Preskill, John",
    title = "{Black holes as mirrors: Quantum information in random subsystems}",
    eprint = "0708.4025",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CALT-68-2659",
    doi = "10.1088/1126-6708/2007/09/120",
    journal = "JHEP",
    volume = "09",
    pages = "120",
    year = "2007"
}

@incollection{halpern2017toward,
  title={Toward physical realizations of thermodynamic resource theories},
  author={Halpern, Nicole Yunger},
  booktitle={Information and Interaction},
  pages={135--166},
  year={2017},
  publisher={Springer}
}

@article{somma2015quantum,
  title={Quantum simulations of one dimensional quantum systems},
  author={Somma, Rolando D},
  journal={arXiv preprint arXiv:1503.06319},
  year={2015}
}

@article{macridin2018digital,
  title={Digital quantum computation of fermion-boson interacting systems},
  author={Macridin, Alexandru and Spentzouris, Panagiotis and Amundson, James and Harnik, Roni},
  journal={Physical Review A},
  volume={98},
  number={4},
  pages={042312},
  year={2018},
  publisher={APS}
}

@article{Garcia-Alvarez:2016wem,
    author = "Garcia-Alvarez, L. and Egusquiza, I.L. and Lamata, L. and del Campo, A. and Sonner, J. and Solano, E.",
    title = "{Digital Quantum Simulation of Minimal AdS/CFT}",
    eprint = "1607.08560",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    doi = "10.1103/PhysRevLett.119.040501",
    journal = "Phys. Rev. Lett.",
    volume = "119",
    number = "4",
    pages = "040501",
    year = "2017"
}

@article{bravyi2002fermionic,
  title={Fermionic quantum computation},
  author={Bravyi, Sergey B and Kitaev, Alexei Yu},
  journal={Annals of Physics},
  volume={298},
  number={1},
  pages={210--226},
  year={2002},
  publisher={Elsevier}
}

@article{Fedichev:2003bv,
    author = "Fedichev, Petr O. and Fischer, Uwe R.",
    title = "{'Cosmological' quasiparticle production in harmonically trapped superfluid gases}",
    eprint = "cond-mat/0303063",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevA.69.033602",
    journal = "Phys. Rev. A",
    volume = "69",
    pages = "033602",
    year = "2004"
}

@article{Fischer:2004bf,
    author = "Fischer, Uwe R. and Schutzhold, Ralf",
    title = "{Quantum simulation of cosmic inflation in two-component Bose-Einstein condensates}",
    eprint = "cond-mat/0406470",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevA.70.063615",
    journal = "Phys. Rev. A",
    volume = "70",
    pages = "063615",
    year = "2004"
}

@article{Obied:2018sgi,
    author = "Obied, Georges and Ooguri, Hirosi and Spodyneiko, Lev and Vafa, Cumrun",
    title = "{De Sitter Space and the Swampland}",
    eprint = "1806.08362",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CALT-TH-2018-020, IPMU18-0100",
    month = "6",
    year = "2018"
}

@article{Russo:2018akp,
    author = "Russo, J. G. and Townsend, P. K.",
    title = "{Late-time Cosmic Acceleration from Compactification}",
    eprint = "1811.03660",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "ICCUB-18-020",
    doi = "10.1088/1361-6382/ab0804",
    journal = "Class. Quant. Grav.",
    volume = "36",
    number = "9",
    pages = "095008",
    year = "2019"
}

@article{Russo:2019fnk,
    author = "Russo, J. G. and Townsend, P. K.",
    title = "{Time-dependent compactification to de Sitter space: a no-go theorem}",
    eprint = "1904.11967",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "ICCUB-19-005",
    doi = "10.1007/JHEP06(2019)097",
    journal = "JHEP",
    volume = "06",
    pages = "097",
    year = "2019"
}

